"Ownership, Not Just Happy Talk": Co-Designing a Participatory Large Language Model for Journalism

Journalism has emerged as an essential domain for understanding the uses, limitations, and impacts of large language models (LLMs) in the workplace. News organizations face divergent financial incentives: LLMs already permeate newswork processes within financially constrained organizations, even as ongoing legal challenges assert that AI companies violate their copyright. At stake are key questions about what LLMs are created to do, and by whom: How might a journalist-led LLM work, and what can participatory design illuminate about the present-day challenges about adapting ``one-size-fits-all'' foundation models to a given context of use? In this paper, we undertake a co-design exploration to understand how a participatory approach to LLMs might address opportunities and challenges around AI in journalism. Our 20 interviews with reporters, data journalists, editors, labor organizers, product leads, and executives highlight macro, meso, and micro tensions that designing for this opportunity space must address. From these desiderata, we describe the result of our co-design work: organizational structures and functionality for a journalist-controlled LLM. In closing, we discuss the limitations of commercial foundation models for workplace use, and the methodological implications of applying participatory methods to LLM co-design.

==> sections/relwork_long.tex <==
\section{Related Works}

Our work sits at the intersection between AI's effect on journalism (\ref{sec:relwork-journ}) and participatory approaches to machine learning (\ref{sec:relwork-participatoryAI}).

% In the related works, we summarize existing work on the tensions and solutions for AI and technology in journalistic practice, and review recent work on participatory approaches to LLMs.

\subsection{AI in journalism}
\label{sec:relwork-journ}

Generative AI has sprawled in influence across the news media ecosystem.
% The sprawling influence of generative AI and LLMs has percolated across the news media ecosystem.
The fundamental new capabilities of these technologies enable the accessible production of naturalistic and inexpensive content, including text, images, and videos.
These new tools hold significant promise for news media~\cite{nishal2024envisioning}, but may also exacerbate existing issues of credibility and authenticity between journalists and their audiences~\cite{toff2024or}.
% These tools produce realistic images, videos, and text, potentially enabling the news media to reach more diverse audiences with relevant content, but also opening up new vulnerabilities.
News organizations have experimented with incorporating various forms of LLMs in their practice, including translating content or improving personalization.
Audiences also increasingly rely on AI-augmented services to access news content, for example through news aggregation platforms like Apple News.
% Audiences are also increasingly using AI to access news content.
Beyond journalists and audiences, AI increasingly mediates the wider ecosystem within which news operates, for example as search platforms like Google and Perplexity produce auto-generated summaries with content gathered from news sources.
% for example in the new introduction of AI-generated summaries on Google and Bing.
% Amidst these complex relationships, 
Finally, the incorporation of AI into these socio-technical systems has proceeded even as concerns around the bias, privacy, and wider ethical implications of these tools remain unresolved~\cite{le2022trust}.

% the use of AI across these systems has also raised new and significant concerns around bias, privacy, and other ethical implications.
% These complex ecosystems have financial stakes, as...
% AI and LLMs have 
% AI and LLMs have changed the way people search for news, how they perceive 

% From upendign search with generative summaries, lowering trust in already-low media through deepfakes, and 

% For decades, journalists have leveraged technology, automation, and AI broadly in journalistic practice.
% Technology, automation, and AI have been deployed by journalists tasks for decades.
% An estimated 82\% of newsrooms use AI in any capacity today, with the leading use cases being the automation of news writing, data analysis, and personalization~\cite{sonni2024digital}.
% Certain types of routine stories, such as earnings reports, weather updates, and sports recaps, have been fully automated in some newsrooms since the early 2000s~\cite{amponsah2024navigating}.
% Nonetheless, recent advances in generative AI models that can emulate natural language on the fly poses a sudden and significant change challenge for the news industry.
% While automated 
% Many parts of the
% This challenge is as much one of perception as tooling...

% In only a few years, LLMs have had specific and significant impacts on journalistic practice.
While flashy as a breakthrough, LLMs are also the latest iteration of a long history of journalists leveraging computing technology, automation, and AI.
% Journalists have leveraged technology, automation, and AI broadly in their work for decades.
% , but LLMs have significantly and suddenly impacted journalistic practice.
% Technology, automation, and AI have been deployed by journalists tasks for decades.
An estimated 82\% of newsrooms use AI today, up from 37\% in 2019, with the leading use cases being the automation of news writing, data analysis, and personalization~\cite{sonni2024digital}.
Such broad adoption of a new technology is remarkable when one considers that journalism has generally been slow to adopt new innovations~\cite{lowrey2011institutionalism}.
Interview studies of journalists adopting machine learning tools in 2019 found that successful use of these tools in newswork requires a delicate balance between maintaining journalistic oversight, developing tool literacy, and honing the technology to work for journalistic tasks~\cite{gutierrez2023question}.
~\citet{jones2022ai} found that while journalists increasingly rely on AI tools throughout their practice, they do not find these systems ``\textit{intelligible};'' there exists a widespread AI literacy problem among media professionals.
% having neither the right perception
% there is an "intelligibility" problems, whereby t
% journalistic understanding of AI technologies lags behind the technology, 
% journalists' understanding of AI tools lags behind the technology, 


Despite these precedents, recent advances in generative AI models that can emulate natural language on the fly stand to significantly impact the news industry.
Although certain types of routine stories, such as earnings reports, weather updates, and sports recaps, have been fully automated for years in many newsrooms~\cite{amponsah2024navigating, beckett2019new}, journalists perceive generative AI as a greater threat to the industry than prior types of automated news writing~\cite{van2024revisiting}.
News organizations have struggled with how to incorporate LLMs into their processes, and have employed a variety of strategies. 
A notable example is that of Sports Illustrated, who outsourced content creation to a third-party vendor that circulated articles created using generative AI and used fake author biographies and pictures, inciting debates about the lack of transparency in AI news reporting~\cite{harrison2023sports}.
% The New York Times took an opposite a
% The BBC (?) meanwhile, has declared that these technologies are not reliable enough in their current form to be used for news writing.
Similarly, Apple News was forced to withdraw a feature that automatically summarized news stories, after the LLM generated false information ~\cite{reilly2025apple}.
These different approaches are likely to have marked impacts on public trust in news, as emerging work finds that news marked as AI-generated is perceived to be less trustworthy~\cite{toff2024or, longoni2022news}.

% These tensions play out differently for heterogeneous newsroom with divergent degrees of data, power, and funding.
% While broad tensions between technology and journalism permeate the industry, 
Significant inter-organizational differences between newsrooms of different sizes and ownership structures also impact journalists' perceptions of technology adoption and use.
Generally speaking, larger and publicly-funded newsrooms are more likely to adopt product innovations~\cite{lowrey2011institutionalism}.
Studies also identified that corporate media ownership may enforce specific technology solutions in an effort to optimize workflows and increase efficiency, which leads to disempowerment and alienation in the workforce~\cite{higgins2021news}.
Meanwhile, journalists in smaller newsrooms often face heightened work stressors, including an increased sense of responsibility towards the community, pervasive job insecurity, and the need to sustain a public-facing persona~\cite{radcliffe2021life, shah2024don, reader2006distinctions}.
Financial stress within smaller news organizations also impacts how new technologies are adopted: the same person is often required to fulfill multiple roles, including being responsible for self-teaching and adopting new technologies with less organizational support~\cite{radcliffe2021life, hoak2021covering}.
In these ways, newsroom size and ownership may also impact the ways that journalists and institutions have the capacity and drive to adopt LLM technologies.
% In a study explicitly focused on newsroom size and ethical comportment, ~\citet{reader2006distinctions} concludes that journalists at smaller newspapers value being accountable to the community, while those at larger newspapers tend to be more attached to their papers' professional reputation.
% When product innovation occurs in large news organizations, these are often a result of 
% Generally speaking, larger newsrooms are more likely to adopt more product innovations, but these are often 
% At larger organizations, innovation within newsrooms has been linekd to enforcement from above~\cite{lowrey2011institutionalism}.

% leading to disempowerment,  


Communication scholars have begun to grapple with how journalists specifically incorporate generative AI and LLMs into their practice.
Through an interview study with journalists, ~\citet{cools2024uses} synthesize a set of ``perils'' (lack of judgment, hallucination and biases, and loss of autonomy) and ``possibilities'' (efficiency and scale, increased personalization) for generative AI in the newsroom.
~\citet{dodds2024impact} identified that knowledge silos, which occur when knowledge is not shared across between roles, teams, and levels of seniority, impeded the effective adoption of AI through limiting shared strategy, know-how, and ethical alignment within organizations. 
Exploring cross-functional collaborations with AI, ~\citet{xiao2024might} found that journalists perceived AI as particularly inaccessible, which necessitates more collaboration with technology companies when out-of-the-box AI tools do not meet journalistic needs and standards.
% presented journalists with a steeper learning curve than prior technologies, 
% Additionally, emergent work posits that 

More technology-oriented academic circles tend to develop specific AI tools for journalistic use cases, and then evaluate them through user studies.
% how specific AI tools can be developed to ease journalistic practice.
For example, tools have been designed and evaluated to aid science journalists~\cite{nishal2024understanding}, scale content audits~\cite{bhargava2024ai, bhargavacase}, and produce short-form video scripts from news stories~\cite{ma2025scrolly2reel, wang2024reelframer}.
These AI-powered tools frequently go beyond existing journalistic practice, for example by proposing new technology-centric mental models for news interactions~\cite{hoque2024towards}.
While these scientific contributions help advance technological innovations, these contributions often hone in on the design of systems and do not always consider the broader socio-technical environment that journalists operate within.


In this paper, we propose an approach to tackle the integration of LLMs in the newsroom that centers financial alignment and governance structures.
This approach fills an important gap and integrates the existing studies we have cited on the technology-forward opportunities of LLMs for journalism and journalists' perception of AI.
We argue that considering financial incentives and governance structures is key to bridging the gap between what is technically feasible, what is organizationally realistic, and what is socially responsible.
As alternative technical governance structures and participation-based models are being developed, there is a need to understand how such a solution could be deployed in the journalistic context.
% Prior work has thus examined potential technical contributions of LLMs for journalism and journalists' perceptions of AI in the newsroom, yet .
% In this study we argue that one area of this puzzle that has heretofore been neglected is the socio-economic lens through which LLMs in journalism may flourish (or perish).
% Due to the often misaligned financial incentives between designers of LLMs and ...

% Specifically, 


% \begin{itemize}

%     \item AI, and particularly large language models, have already had a significant impact on the media ecosystem. LLMs have changed the way people find and receive media.  For example, LLMs built into search engines like Google pull out snippets from articles, stopping traffic from ever reaching a news org's webpage.  [cite Felix Simon's paper]
%     \item AI has also impacted journalistic practice. Journalists have been using various forms of AI for years for tasks like newsgathering and templating.
%     \item However, the relatively more recent emergence of LLMs have caused outlets to contend with how to adopt them in their process. Talk about a few approaches (e.g. NYTimes author bylines), maybe also scandals (e.g. Sports Illustrated). Companies have adopted specific rules. Some have leaned in and some haven't. Even beyond what is officially adopted by companies, individual journalists are increasingly using AI, e.g. ~\cite{xiao2024might}
%     \item These tensions also stand to impact different newsrooms heterogeneously.
%     \item Comm scholars have focused on journalist experiences and use of AI in practice...
%     \item Technical conferences have largely focused on AI tooling for journalists... (talk about examples)
%     \item We bridge this research gap with a socio-technical investigation of... : As alternative and participation-based models are being developed, there is a need to understanding how such a solution could be deployed in this context.
% \end{itemize}

\subsection{Participation and ownership in LLMs}
\label{sec:relwork-participatoryAI}

The development of LLMs, as well as the compilation and storage of the datasets they are trained on, is heavily centralized within large corporations \cite{luitse2021great}.  Downstream applications and/or users must accept the pretrained model as is, without control over or transparency into data sources, underlying design decisions, fine-tuning or alignment procedures, and future data or model changes.  For example, a small business using a tool built on top of a proprietary, general-purpose foundation model has little ability to understand whether the data practices of the model align with their values, and little leverage to push for any changes regardless.  While open-source models are seemingly more transparent, it is typically only model weights that are released, not datasets; and the sheer size of such models renders them difficult to actually examine by most without access to significant compute resources \cite{widder2024open}. 

Recent work has recognized the importance of \textit{participatory} approaches in response to power imbalances in AI more broadly \cite{delgado2023participatory}.  Here, we particularly draw on bodies of participatory scholarship that are focused on distributing power to those who typically do not have it \cite{arnstein1969ladder,birhane2022power,corbett2023power}.  Work in participatory AI has characterized a spectrum of approaches, from those that take a more tokenistic approach (e.g., one-time user feedback that shapes model fine-tuning) to those that attempt to meaningfully share decision-making power (e.g., sustained relationships with affected communities who are involved in many project stages, from data collection to evaluation) \cite{sloane2022participation}.  LLMs introduce unique challenges for participatory approaches that aim to distribute decision-making power, due to their centralized and largely corporate control \cite{suresh2024participation}.  To support more meaningful participation in this ecosystem, \citet{suresh2024participation} propose a domain-specific ``subfloor'' that builds on a foundation model.  The subfloor encompasses ``technical infrastructure, norms, and governance for a grounded domain,'' aiming to support more tractable participation grounded in the needs and stakeholders of a specific context.  This paper takes inspiration from the idea of a subfloor for journalism---an industry-wide collective that might support the creation of licensable datasets, shared models/tools, AI policies and best practices, or more.  Through interviews with journalists across varied roles and organizations, we draw out concrete opportunities and challenges for actually building out this kind of collective organization for developing, maintaining and/or governing LLMs in the news industry.   
